BadFusion: 2D-Oriented Backdoor Attacks against 3D Object Detection

3D object detection plays an important role in autonomous driving; however, its vulnerability to backdoor attacks has become evident. By injecting ''triggers'' to poison the training dataset, backdoor attacks manipulate the detector's prediction for inputs containing these triggers. Existing backdoor attacks against 3D object detection primarily poison 3D LiDAR signals, where large-sized 3D triggers are injected to ensure their visibility within the sparse 3D space, rendering them easy to detect and impractical in real-world scenarios. In this paper, we delve into the robustness of 3D object detection, exploring a new backdoor attack surface through 2D cameras. Given the prevalent adoption of camera and LiDAR signal fusion for high-fidelity 3D perception, we investigate the latent potential of camera signals to disrupt the process. Although the dense nature of camera signals enables the use of nearly imperceptible small-sized triggers to mislead 2D object detection, realizing 2D-oriented backdoor attacks against 3D object detection is non-trivial. The primary challenge emerges from the fusion process that transforms camera signals into a 3D space, compromising the association with the 2D trigger to the target output. To tackle this issue, we propose an innovative 2D-oriented backdoor attack against LiDAR-camera fusion methods for 3D object detection, named BadFusion, for preserving trigger effectiveness throughout the entire fusion process. The evaluation demonstrates the effectiveness of BadFusion, achieving a significantly higher attack success rate compared to existing 2D-oriented attacks.

==> BP_folder/AuthorFeedbackFinal.tex <==
\noindent We appreciate all reviewers' constructive feedback and recognition of our strengths, such as ``work is novel,'' ''timely and relevant,'' ``experiments are comprehensive,'' ``paper is written well.'' We hope the following clarifications will satisfactorily address the concerns raised by reviewers.

\vspace{0.3em}
\noindent\textbf{To Reviewer \#1:} \vspace{0.3em}

\noindent
\textbf{Q1.  For the disappear attack, why is it easier to remove the bounding box for closer objects than the farther objects?} %

\noindent As described in the paper, to implement disappear attacks, we shift the center coordinates of the bounding boxes in the poisoned data either closer to or farther from the target vehicle. These modifications are classified as disappear attack (closer) and disappear attack (farther).
Our experiments have revealed that learning of disappear attack (farther) is more challenging than the learning disappear attack (closer) for the poisoned model. This challenge arises particularly when the vehicle with a backdoor trigger is very close to the target vehicle in the scene. %
Even if its corresponding bounding box is relocated far away during the poisoning process of the disappear attack (farther), it might still occasionally appear in the scene. 
Such occurrences inadvertently teach the model far bounding box attack behavior instead of disappearing attack, which can interrupt the learning process of the disappearing attack during the training of the poisoned model. %
As a result, the disappear attack (farther) yields a lower Attack Success Rate (ASR) than the disappear attack (closer).

\vspace{0.3em}
\noindent\textbf{To Reviewer \#2:} \vspace{0.3em}

\noindent
\textbf{Q1. Clarify the paper’s focus in the introduction section.} 

\noindent We appreciate this suggestion and will clarify our focus on fusion-based object detection approaches at the beginning of the introduction section. %

\vspace{0.1em}
\noindent\textbf{Q2. What fusion models are used in Tables 2, 3, and 4? Is “uniform color” equivalent to “solid color” in the paper?}

\noindent This paper considers the MVX-Net fusion method in Tables 2, 3, and 4, which will be updated in table captions for clarification. Furthermore, we acknowledge that "uniform color" and "solid color" are equivalent in this paper. We sincerely appreciate your attention to this inconsistency and will make corrections throughout the paper.

\vspace{0.1em}
\noindent\textbf{Q3. Discussion on why the trigger sizes do not significantly impact the attack performance.}

\noindent In the section ``Impact of Trigger Size and Poisoning Rate" in the ablation study, we observe that increasing the trigger size does not necessarily improve attack performance. Specifically, Figure~\ref{fig:pr_ts} illustrates that the range of effective trigger pixels for a trigger size of $15 \times 15$ varies from 0 to 60, with a primary range of 25 to 35. %
In contrast, for a trigger size of $20 \times 20$, the range of effective trigger pixels varies from 0 to 80, with a primary range of 38 to 55.
Therefore, the small range of effective trigger pixels for trigger size %
results in a more consistent trigger pattern across samples in the training and inference phases, leading to a better attack performance. %
This will be clarified in the corresponding section. 

\vspace{0.1em}
\noindent\textbf{Q4. %
It would be interesting to investigate the cases where the attack fails.}

\noindent We value Reviewer 2's interest in exploring scenarios where the proposed attack might fail. We have identified the failure cases arising from two main issues: 1) \textit{sparse trigger locations}, where the projection of LiDAR signals lacks sufficient points to transform sufficient trigger points, even after identifying a dense location, and 2) \textit{overlapping trigger locations}, although the proposed BadFusion inserts the trigger at the densest LiDAR point locations during the poisoning process, if the trigger is placed in a region where the bounding boxes of two vehicles overlap during inference, the poisoned model might either predict a reduced-size bounding box or no detection for this unintended neighboring vehicle (assuming the trigger is present for that vehicle). A potential solution to mitigate this issue is to avoid inserting triggers in areas of bounding box overlap during the inference phase.

\vspace{0.3em}
\noindent\textbf{To Reviewer \#4:} \vspace{0.3em}

\noindent\textbf{Q1. What are the reasons that OptimizedTrigger and UntarOD perform better on the EPNet fusion method, and does it work better for EPNet++?}  %

\noindent We appreciate Reviewer 4's insightful suggestion. We believe the fusion manner proposed in EPNet plays a critical role in its vulnerability to backdoor attacks. To enhance the correspondence between the camera and LiDAR features, EPNet first uses LiDAR features to guide the image features before the camera-LiDAR fusion, named LiDAR-guided Image Fusion (LI-Fusion), and then generates point-wise image features. Here, a bilinear interpolation-based image sampler is applied for each LiDAR point to extract neighboring image features. Thus, despite the lack of corresponding LiDAR points, the backdoor triggers injected in the 2D camera space can still be learned through the neighboring LiDAR points during the interpolation process. This eliminates the sparsity challenges in existing 2D-oriented backdoor attacks, such as OptimizedTrigger and UntarOD.
Therefore, as shown in the results, the performance of existing attacks on EPNet is higher than that of other fusion methods, such as MVX-Net and Focals-ConvF.
It should be mentioned that the proposed BadFusion attack is effective in various fusion methods, such as MVX-Net, Focals Conv-F, and EPNet. In contrast, the existing attacks are effective only when backdoor triggers are activated in the fusion, e.g., through interpolation in EPNet.
We will clarify the reason in the revision.
 
Additionally,  we believe the Cascade Bi-directional Fusion (CB-Fusion) module proposed in EPNet++ could further enhance the impact of backdoor triggers. In CB-Fusion, following the LI-fusion, Image-guided LiDAR Fusion (IL-Fusion) is developed to LiDAR features by image features. Specifically, the image features learned by LI-Fusion will be used to guide the generation of LiDAR features, and thus the backdoored image features presented in EPNet could affect the LiDAR features. Therefore, the CB-Fusion could further amplify the backdoor attacks in EPNet++. We will conduct additional experiments to verify this. 


\vspace{0.1em}
\noindent\textbf{Q2. It would be better if the section of related works could be put before Section 2.} 

\noindent We appreciate this valuable suggestion and will reorganize the paper to improve the paper's logic.


